Finding Locally Densest Subgraphs: Convex Programming with Edge and Triangle Density

Finding the densest subgraph (DS) from a graph is a fundamental problem in graph databases. The DS obtained, which reveals closely related entities, has been found to be useful in various application domains such as e-commerce, social science, and biology. However, in a big graph that contains billions of edges, it is desirable to find more than one subgraph cluster that is not necessarily the densest, yet they reveal closely related vertices. In this paper, we study the locally densest subgraph (LDS), a recently proposed variant of DS. An LDS is a subgraph which is the densest among the ``local neighbors''. Given a graph $G$, a number of LDSs can be returned, which reflect different dense regions of $G$ and thus give more information than DS. The existing LDS solution suffers from low efficiency. We thus develop a convex-programming-based solution that enables powerful pruning. We also extend our algorithm to triangle-based density to solve LTDS problem. Based on current algorithms, we propose a unified framework for the LDS and LTDS problems. Extensive experiments on thirteen real large graph datasets show that our proposed algorithm is up to four orders of magnitude faster than the state-of-the-art.

==> exp.tex <==
%!TEX root = ./main.tex
\color{black}
\section{Experiments}
\label{sec:exp}
% In this section, we present the experimental results. 
%We first give the experiment setup in \Cref{sec:exp:setup}. \Cref{sec:exp:efficiency,sec:exp:memory} give the comparison between our {\tt LDScvx} and the state-of-the-art {\tt LDSflow} on running time and memory usage, respectively. \Cref{sec:exp:proportion,sec:exp:ablation} present the detailed analysis over different components on our algorithm. We give the LDS statistics over different datasets in \Cref{sec:exp:lds-stat} and a case study over a movie dataset in \Cref{sec:exp:case-study}.

\subsection{Setup}
\label{sec:exp:setup}

We use nine real datasets \cite{snapnets,nr,yang2015defining,boldi2011layered,boldi2004webgraph} which are publicly available\footnote{\url{https://networkrepository.com/}, \url{https://snap.stanford.edu/data/index.html}, and \url{https://law.di.unimi.it/datasets.php}} except for TL. The TL dataset is provided by a television company TCL Technology. The dataset contains film information provided on its smart TV platform, mainly used for a case study. Other graph datasets cover various domains, including social networks (e.g., LiveJournal), e-commerce (e.g., Amazon), and video platforms (e.g., YouTube). \Cref{tab:datasets} summarizes the statistics.
% Table generated by Excel2LaTeX from sheet 'datasets'
\begin{table}[htbp]
    \centering
    \caption{Graphs used in our experiments.}
    \algofont
    \begin{tabular}{l|l|l|r|r}
        \hline
        Dataset & Full name       & Category      & $|V|$ & $|E|$ \\
        \hline
        \hline
        TL      & movie-TCL       & Movie         & 108K  & 168K  \\
        \hline
        AM      & com-amazon      & E-commerce    & 335K  & 926K  \\
        \hline
        YT      & com-youtube     & Video-sharing & 1.13M & 2.99M \\
        \hline
        LJ      & com-lj          & Social        & 4.00M & 34.7M \\
        \hline
        OR      & com-orkut       & Social        & 3.07M & 117M  \\
        \hline
        \MD{IC} & indochina-2004  & web           & 7.41M & 194M  \\
        \hline
        \MD{AB} & arabic-2005     & web           & 22.7M & 639M  \\
        \hline
        IT      & web-it-2004-all & Web           & 41.3M & 1.03B \\
        \hline
        LK      & links-anon      & Hyperlink     & 52.6M & 1.61B \\
        \hline
    \end{tabular}%
    \label{tab:datasets}%
\end{table}%

We compare the following LDS algorithms:
\begin{itemize}[leftmargin=*]
    \item {\tt LDScvx} is our convex-programming based top-$k$ LDS algorithm (\Cref{sec:algo:lds}).
    \item {\tt LDSflow} \cite{qin2015locally} is the state-of-the-art top-$k$ LDS algorithm based on max-flow.
\end{itemize}

% Note that the parameter $N$ of \FW is set to 100, which is the number of iterations. 
All the algorithms above are implemented in C++ with STL used. The source codes of {\tt LDSflow} are provided by the authors of \cite{qin2015locally}. We run all the experiments on a machine having an Intel(R) Xeon(R) Silver 4110 CPU @ 2.10GHz processor and 256GB memory, with Ubuntu installed.

\subsection{Efficiency Results}
\label{sec:exp:efficiency}

\MD{To choose the best setting of $N$, i.e., the number of \FW iterations, we tested the running time of {\tt LDScvx} w.r.t. different values of $N$ from 50 to 200 with $k$ fixed to $5$. \Cref{tab:para-N} reports the average relative running time w.r.t. $N$ over eight large datasets. The relative running time for a specific value of $N$ on each dataset is obtained via dividing the running time by the minimum running time over all $N$ values for the dataset. The mean is then obtained by averaging over all datasets. We can find that when $N=100$, we obtain the minimum average relative running time. Hence we use $N=100$ as the default parameter value in other experiments.}

\begin{table}[htbp]
    \centering
    \caption{\MD{Relative running time w.r.t. different $N$}}
    \begin{tabular}{r|r|r|r|r}
        \hline
        $N$                   & 50   & 100  & 150  & 200  \\
        \hline
        \hline
        Average relative time & 1.64 & 1.10 & 1.12 & 1.20 \\
        \hline
    \end{tabular}%
    \label{tab:para-N}%
\end{table}%


Next, we compare our top-$k$ LDS algorithm {\tt LDScvx} with the state-of-the-art {\tt LDSflow} \cite{qin2015locally} w.r.t. running time.

\begin{figure}[htb]
    \input{figs/time-overall}
    \vspace{-1em}
    \caption{Efficiency of {\tt LDScvx} and {\tt LDSflow} with $k=5$.}
    \label{fig:eff-overall}
\end{figure}

We first fix $k=5$ to overview the two algorithms on the nine datasets w.r.t. running time. \Cref{fig:eff-overall} shows the efficiency results of the two algorithms. The datasets are ordered by graph size on the x-axis. Note that for some datasets, the bars of {\tt LDSflow} touch the solid upper line, which means {\tt LDSflow} cannot finish within 600 hours on those datasets. From \Cref{fig:eff-overall}, we can observe: first, the running time of {\tt LDSflow} increases along with the graph size increasing; second, {\tt LDScvx} is up to four orders of magnitude faster than {\tt LDSflow}. We reckon that the speedup comes from \MD{more vertices pruned due to tighter bounds, fewer LDS candidates verified, and smaller flow networks as stated in \Cref{sec:algo}.}
% \begin{enumerate*}
%   \item tighter upper and lower bounds of compact numbers provided by $\mathsf{CP}(G)$ helps prune more vertices;
%   \item smaller subgraphs involved for LDS verification by \Cref{thm:isLDS} reduce the computation cost of max-flow.
% \end{enumerate*}

\begin{figure}[htb]
    \input{figs/time-k}
    \vspace{-1em}
    \caption{Efficiency of {\tt LDScvx} and {\tt LDSflow} w.r.t. different $k$.}
    \label{fig:eff-k}
\end{figure}

We further provide the running time trends of the two algorithms w.r.t. different $k$ values on \MD{four representative datasets in \Cref{fig:eff-k} due to space limit}. For {\tt LDSflow}, we do not show its trends on dataset LK because it cannot finish within 600 hours even with $k=5$. We can see that when $k$ increases, the running time of both {\tt LDScvx} and {\tt LDSflow} increases. Furthermore, there is a significant increase in {\tt LDSflow} (about two orders of magnitude) when $k$ is increased from $10$ to $15$ on dataset YT. To analyze this significant surge, we examine the running process of the two algorithms. We found that many LDS candidates in {\tt LDSflow} do not pass the verification process when $k$ is increased from $10$ to $15$. Recall that {\tt LDSflow} needs to perform max-flow computation on a flow network to verify each LDS candidate according to \Cref{sec:algo:verify}. Hence, the number of failed LDS candidates can reveal to some extent the reason of the spike in running time.

% Table generated by Excel2LaTeX from sheet 'failed YT'
\begin{table}[htbp]
    \centering
    \caption{Numbers of failed LDS candidates on YT w.r.t. $k$.}
    \begin{tabular}{l|r|r|r}
        \hline
        Algorithm     & $k=10$ & $k=15$ & increased times \\
        \hline
        \hline
        {\tt LDScvx}  & 37     & 84     & 2.27$\times$    \\
        \hline
        {\tt LDSflow} & 277    & 18399  & 66.42$\times$   \\
        \hline
    \end{tabular}%
    \label{tab:failed-YT}%
\end{table}%

We report the numbers of failed LDS candidates on YT with $k=10$ and $15$ for both algorithms in \Cref{tab:failed-YT}. We observe that the number of failed candidates in {\tt LDSflow} increased around 66$\times$ when $k$ increases from $10$ to $15$, which explains the surge of running time in \Cref{fig:eff-k}. In contrast, the number of failed candidates in {\tt LDScvx} only increases by about 2$\times$. This is why the running time of {\tt LDScvx} does not increase much when $k$ is increased from 10 to 15. Another observation from \Cref{tab:failed-YT} is that the failed numbers for {\tt LDScvx} are smaller than {\tt LDSflow} on both $k$ values, respectively. The reason is that we provide tight upper and lower bounds for compact numbers via convex programming and stable groups, and the tight bounds further enable more vertices to be pruned, which results in fewer LDS candidates to be examined. Apart from that, to examine an LDS candidate, our {\tt LDScvx} only needs a subgraph of what is needed in {\tt LDSflow} to calculate the max-flow by leveraging the lower bounds of compact numbers, according to \Cref{sec:algo:verify}. We believe the above two improvements explain why we are around three orders of magnitude faster on YT when $k=15$.

\MD{We further tested the scalability w.r.t. the density via synthetics datasets. The six synthetic graphs are generated by Barab\'{a}si-Albert (BA) model \cite{albert2002statistical}. The numbers of vertices in all synthetic graphs are fixed to 1,000,000, and the densities are increased linearly from 2 to 12. In other words, the numbers of edges are from 2,000,000 to 12,000,000. We report the running time of {\tt LDScvx} on the six synthetic datasets in \Cref{fig:scalability}. We observe that {\tt LDScvx} scales well w.r.t. the graph density.}

\begin{figure}[h]
    \input{figs/synthetic.tex}
    \vspace{-1em}
    \caption{\MD{The scalability w.r.t. the density.}}
    \label{fig:scalability}
\end{figure}


\subsection{Memory Usage Comparison}
\label{sec:exp:memory}
In this subsection, we test the memory usage of the two algorithms. The maximum memory usage is tested via the Linux command {\tt /usr/bin/time -v}. For the cases that {\tt LDSflow} does not finish reasonably, we record the maximum resident memory during the running process.
\Cref{fig:memory} reports the maximum memory usage of the two algorithms. The datasets are sorted on the x-axis in ascending order of graph size. We can observe that the memory usages of both algorithms increase along with the increasing graph size. Besides, the memory costs of {\tt LDScvx} and {\tt LDSflow} are around the same scale because the two algorithms take linear memory usage w.r.t. the graph size.

\begin{figure}[htb]
    \input{figs/memory-usage}
    \vspace{-1em}
    \caption{Memory usage of algorithms with $k=5$.}
    \label{fig:memory}
\end{figure}

\subsection{Time Proportion Analysis}
\label{sec:exp:proportion}

\begin{figure}[htbp]
    \input{figs/time-proportion}
    \vspace{-1em}
    \caption{Proportion of each part in total running time.}
    \label{fig:time-proportion}
\end{figure}

Here, we evaluate how the different building blocks of {\tt LDScvx} contribute to the whole running time after the graph is loaded and preprocessed. \Cref{fig:time-proportion} reports the proportion of each part in the total running time: Frank-Wolfe (\Cref{alg:fw}), ExtractSG (\Cref{alg:ext-sg}), Pruning (\Cref{alg:pruning}), and VerifyLDS (\Cref{alg:is-lds}) with $k=5$ over nine datasets. We can observe that the Frank-Wolfe computation is the most computationally expensive part on most datasets. For LK and YT datasets, the time used by verifying LDS takes the majority. We further examine the number of failed LDS candidates (i.e., on which \IsLDS returns {\sf False}) on the nine datasets. \Cref{tab:failed-can} reports the results. We can find that the numbers of failed candidates on LK and YT are much higher than other datasets, which means that these two datasets need more time to verify LDS's, which explains the results in \Cref{fig:time-proportion} to some extent. \MD{For IC, the time used by verifying LDS is also high, because the first LDS in IC is quite large and takes relatively long time to verify.}

% Table generated by Excel2LaTeX from sheet 'filed candidate'
\begin{table}[htbp]
    \centering
    \caption{Numbers of failed LDS candidates with $k=5$.}
    \algofont
    \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
        \hline
        Dataset  & TL & AM & YT & LJ & OR & \MD{IC} & \MD{AB} & IT & LK \\
        \hline
        \hline
        \#failed & 1  & 0  & 9  & 1  & 1  & 0       & 0       & 0  & 6  \\
        \hline
    \end{tabular}%
    \label{tab:failed-can}%
\end{table}%

\subsection{Ablation Study of {\tt IsLDS}}
\label{sec:exp:ablation}
Here, we conduct an ablation study on {\tt LDScvx} to understand the effectiveness of {\tt IsLDS} (\Cref{alg:is-lds}). Recall that in {\tt IsLDS} we only include the vertices satisfying $\overline{\phi}(u) \geq \mathsf{density}(G[S]) \geq \underline{\phi}(u)$ into the flow network computation, while its counterpart in {\tt LDSflow} \cite{qin2015locally} includes all vertices satisfying $\overline{\phi}(u) \geq \mathsf{density}(G[S])$, named by {\tt IsLDS-ab} (ablation). We report the time used for verifying LDS's with {\tt IsLDS} and {\tt IsLDS-ab}, respectively, on the nine datasets when $k=5$ in \Cref{tab:ablation}. \MD{Here, the time of {\tt IsLDS-ab} is measured by replacing {\tt IsLDS} with {\tt IsLDS-ab} in {\tt LDScvx}.} The time of {\tt IsLDS-ab} on LK is marked as $\geq 259200$s because it cannot finish within three days. From the results, we observe that the verification process with {\tt IsLDS} is up to 110$\times$ faster than that with {\tt IsLDS-ab}. Hence, reducing the number of vertices by the lower bounds in {\tt IsLDS} does help speed up the LDS verification process.

% Table generated by Excel2LaTeX from sheet 'ablation'
% \begin{table}[htbp]
%   \centering
%   \caption{Effect of {\tt IsLDS} with $k=5$}
%   \algofont
%     \begin{tabular}{l|r|r|r|r|r|r}
%     \hline
%     Dataset & AM & YT & LJ & OR & IT & LK \\
%     \hline
%     {\tt IsLDS} & 0.33s & 2.7s & 2.1s & 18s & 148s & 2335s \\
%     \hline
%     {\tt IsLDS-ab} & 0.36s & 81s & 2.4s & 724s & 189s & NA \\
%     \hline
%     Speedup & 1.09 & 30.48 & 1.13 & 39.31 & 1.28 & NA \\
%     \hline
%     \end{tabular}%
%   \label{tab:ablation}%
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'ablation'
\begin{table}[htbp]
    \centering
    \caption{Effect of {\tt IsLDS} with $k=5$.}
    \begin{tabular}{l|r|r|r}
        \hline
        Dataset & {\tt IsLDS} & {\tt IsLDS-ab} & Speedup             \\
        \hline
        \hline
        TL      & 0.0399s     & 0.0748s        & $1.87\times$        \\
        \hline
        AM      & 0.3334s     & 0.3623s        & $1.09\times$        \\
        \hline
        YT      & 2.6575s     & 80.9994s       & $30.48\times$       \\
        \hline
        LJ      & 2.1204s     & 2.3924s        & $1.13\times$        \\
        \hline
        OR      & 18.4089s    & 723.6035s      & $39.31\times$       \\
        \hline
        \MD{IC} & 285.4502s   & 288.9184s      & $1.01\times$        \\
        \hline
        \MD{AB} & 60.2669s    & 62.0416s       & $1.03\times$        \\
        \hline
        IT      & 147.9361s   & 188.8527s      & $1.28 \times$       \\
        \hline
        LK      & 2335.4461s  & $\geq 259200$s & $\geq 110.99\times$ \\
        \hline
    \end{tabular}%
    \label{tab:ablation}%
\end{table}%


\subsection{Subgraph Statistics}
\label{sec:exp:lds-stat}

% In this subsection, we report the densities of the top-15 LDS's with respect to the size (number of vertices) of each LDS on the six large datasets. We show the statistics in \Cref{fig:density-size}. We can find that the statistic patterns look different among different datasets. For example, the LDS's in AM have quite close densities around 4.7. There is only one LDS for OR, so there is only one triangle in the plot center. For LJ and IT, the LDS's have relatively wide ranges of density and size, respectively. For YT and LK, there are a large LDS and many small LDS's (the points of smaller LDS's in LK overlap in the left bottom corner), so their plots look similar. Recall that the top-1 LDS (i.e., the densest LDS) is also the DS of the graph. Hence, we can find that the LDS model can provide some smaller and handy subgraphs than DS, which may help users explore.
%The plots can mean that there are many relatively small dense regions in AM, while there is a certain large dense region in LK. 

\MD{In this subsection, \Cref{fig:density-size} reports the densities of the top-15 densest subgraphs w.r.t. the size (number of vertices) returned by three different models on four datasets, where {\tt Greedy} iteratively computes a densest subgraph and removes it from the graph, and {\tt FDS} denotes the density-friendly decomposition model \cite{tatti2015density,danisch2017large}. From \Cref{fig:density-size}, we can find that the densest subgraph can be found by all three algorithms, because the densest subgraph is also an LDS. But there are some  dense subgraphs found by {\tt Greedy} that do not qualify as LDS's. Hence, the subgraphs found by {\tt LDScvx} have a wide range of densities and sizes. For {\tt FDS}, we can find that the subgraphs have increasing sizes and decreasing densities. This is because {\tt FDS} outputs a chain of subgraphs, where each subgraph is nested within the next one, and the inner one is denser than the outer ones.}

\begin{figure}[htb]
    \input{figs/density-size2}
    \vspace{-1em}
    \caption{Subgraph statistics: density w.r.t. size.}
    \label{fig:density-size}
\end{figure}

% The density-size plots (\Cref{fig:density-size}) give us an overall picture of the LDS's in different datasets. 
% Next, we will use a case study to see what an LDS looks like concretely in the following subsection.

\subsection{Case Study}
\label{sec:exp:case-study}

Here, we perform a case study on the TL dataset. The TL dataset is provided by a Chinese television company, TCL Technology, which contains three types of vertices: director, movie, and actor.

% \begin{figure}[htb]
% \includegraphics[width=0.48\textwidth]{figs/untra-seven.pdf}
% \caption{A movie community about ``Ultraman''.}
% \label{fig:case-study}
% \end{figure}

After examining the top-10 LDS's returned by our LDS algorithm, we found that the LDS's on the TL dataset are about different topics. For example, \Cref{fig:case-study} shows the LDS with the third-highest density. This LDS contains eight movies related to a famous Japanese sci-fiction series ``Ultraman'' with four actors and one director. In this LDS, the four actors participated in all eight films, and the director directed five of them.
The LDS with the second-highest density is a subgraph about Chinese martial fiction. Other LDS's cover topics about western films, Danish comedies, and cartoons, while the DS model can only find a large subgraph about western films.
% \MD{We have also examined the top-10 subgraphs with highest densities by {\tt FDS} \cite{danisch2017large}. We found that the subgraphs are mainly about western films and Chinese fictions.} 
Hence, from the output of the case study, we reckon that the subgraphs returned by the LDS algorithm are good representations of {\em different} local dense regions in the graph.







==> figs/conc.tex <==
%!TEX root = ./main.tex

\section{Conclusion}
\label{sec:conc}
In this paper, we study the problem of finding the top-$k$ locally densest subgraphs (LDS's) in a graph for identifying the local dense regions from the graph. The LDS's are usually compact and dense. To facilitate the LDS discovery, we propose a new concept, named {\em compact number} for each vertex, which denotes the compactness of the most compact subgraph containing the corresponding vertex. By leveraging the compact number and its relations with the LDS problem and a specific convex program, we derive a convex-programming based algorithm {\tt LDScvx} following the pruning-and-verify paradigm.
For pruning, we derive tight upper and lower bounds of compact numbers and design powerful pruning techniques based on the bounds.
For verification, we minimize the size of the subgraph needed for max-flow computation via further exploiting the lower bounds of compact numbers.
Extensive experiments on six datasets show that {\tt LDScvx} is up to four orders of magnitude faster than the state-of-the-art algorithm.
The case study performed on a movie dataset reveals that the output subgraphs by our LDS algorithm are high-quality representations of local dense regions of the graph.

In the future, it is interesting to see whether the LDS model can be extended to other graph types, e.g., bipartite graphs and directed graphs. Besides, extending the edge-based density to clique-based density for the LDS problem is also worth investigating.
